On the privacy-utility trade-off in differentially private hierarchical text classification

Hierarchical text classification consists in classifying text documents into a hierarchy of classes and sub-classes. Although artificial neural networks have proved useful to perform this task, unfortunately they can leak training data information to adversaries due to training data memorization. Using differential privacy during model training can mitigate leakage attacks against trained models, enabling the models to be shared safely at the cost of reduced model accuracy. This work investigates the privacy-utility trade-off in hierarchical text classification with differential privacy guarantees, and identifies neural network architectures that offer superior trade-offs. To this end, we use a white-box membership inference attack to empirically assess the information leakage of three widely used neural network architectures. We show that large differential privacy parameters already suffice to completely mitigate membership inference attacks, thus resulting only in a moderate decrease in model utility. More specifically, for large datasets with long texts we observed Transformer-based models to achieve an overall favorable privacy-utility trade-off, while for smaller datasets with shorter texts convolutional neural networks are preferable.

==> src/evaluation.tex <==
\section{Reference datasets}
\label{sec:data}

We consider three real-world datasets: the BestBuy dataset, which represents a consumer product hierarchical classification task; the Reuters dataset, which contains news articles; and the DBPedia dataset with Wikipedia excerpts. The datasets have varying text lengths (34 to 212 words), differ in the number of overall data (51,000 to 800,000 records) and have also been used in related work on HTC without DP and MI.
\\
\\
\textbf{BestBuy.} The BestBuy dataset\footnote{\url{https://github.com/BestBuyAPIs/open-data-set}} contains $51,646$ unique products, each consisting of categorical features (e.g., SKU, type, manufacturer), numerical features such as price, textual features (e.g., name, description) and URLs, that are composed of one or more of the aforementioned features. Training a differentially private HTC model on datasets like BestBuy can therefore prevent leaking sensitive information about individual products of a company. 

In our experiments, we concatenate the features \enquote{name}, \enquote{manufacturer} and \enquote{description} to a single string and ignore the other features for classification. This selection is based on empirically observed superior classification accuracy. On average, the resulting concatenated texts have a length of 34 words. Additionally, every product holds a special feature called \enquote{category} assigning the product to a \textit{single}, \textit{partial-depth} class label in the BestBuy product hierarchy. 

The BestBuy product hierarchy is a \textit{tree} and consists of seven levels, each with a different number of classes, as shown in Table~\ref{tab:dataset-hierarchy}. As can be seen, level $L_4$ has the most classes. Also, we can see that even on the first level, not all of the existing $51,646$ products are assigned to a class. Particularly, we found that 256 products ($0.50$\%) are assigned to classes not contained in the BestBuy product hierarchy. We removed these products as the assigned classes did not fit into the given product hierarchy (e.g., \enquote{Other Product Categories} or \enquote{In-Store Only}). Furthermore, not every product is assigned to a class on every level, meaning the most specific class of many products is on a lower level than $L_7$. In our experiments, we only make use of the first three hierarchy levels. We decided to do so due to the long tail characteristic of the dataset. Thus, the predictions of our classifiers are less specific than potentially possible, but more robust due to a higher number of training examples in comparison to fine grained training for all hierarchies. 10\% of the overall data was used for testing.

All datasets have been \emph{tokenized}, which means that the text has to be split up into a sequence of smaller units called \emph{tokens}. A natural tokenization technique is splitting the text into a sequence of words,so that each token represents a word. After tokenization, the token sequence is converted into an integer sequence since ANNs only take numbers as input. During the conversion, a vocabulary is created that maps each token to a unique integer so that the same token is always converted into the exact same integer. The size of the vocabulary then represents the number of unique tokens in the text.
\begin{table}[ht!]
\centering
\begin{tabular}{c|c|c|c}
Hierarchy Level & Dataset & Classes & Assigned products \\ \hline
\multirow{3}{*}{Level $L_1$} & BestBuy & $19$ & $51,390$ \\ \cline{2-4} 
 & DBPedia & $9$ & $337,739$ \\ \cline{2-4} 
 & Reuters & $4$ & $804,427$ \\ \hline
\multirow{3}{*}{Level $L_2$} & BestBuy & $164$ & $50,837$ \\ \cline{2-4} 
 & DBPedia & $70$ & $337,739$ \\ \cline{2-4} 
 & Reuters & $55$ & $779,714$ \\ \hline
\multirow{3}{*}{Level $L_3$} & BestBuy & 612 & $44,949$ \\ \cline{2-4} 
 & DBPedia & 219 & $337,739$ \\ \cline{2-4} 
 & Reuters & 43 & $406,961$ \\ \hline
Level $L_4$ & BestBuy & $771$ & $26,138$ \\ \hline
Level $L_5$ & BestBuy & $198$ & $5,640$ \\ \hline
Level $L_6$ & BestBuy & $23$ & $346$ \\ \hline
Level $L_7$ & BestBuy & $1$ & $1$ \\
\end{tabular}
    \caption{Classes and assigned records per level per dataset.}
    \label{tab:dataset-hierarchy}
\end{table}
\\
\\
\textbf{Reuters Corpus Volume 1.} The \enquote{Reuters Corpus Volume 1} (RCV1) dataset\footnote{\url{https://trec.nist.gov/data/reuters/reuters.html}} is an archive of over $800,000$ manually categorized news articles~\cite{lewisRCV1NewBenchmark2004}. Per news article, a headline, text block and topic codes representing the classes in the hierarchy are provided. In our experiments we use the concatenation of headline and text block as input for the respective classifiers. The resulting texts have an average length of 237 words. Table~\ref{tab:dataset-hierarchy} shows the number of classes and assigned documents for each hierarchy level of the Reuters dataset. To ensure comparability with state of the art we follow the approach of Stein et al.~\cite{steinAnalysisHierarchicalText2019} and randomly assign $80,443$ texts to the test dataset and assign each news article to the least frequent topic code. This approach is based on the assumption that the least common topic code is the one that most specifically characterizes the document. A differentially private HTC model trained on a non-public article dataset such as RCV1 can prevent leaking sensitive information represented by individual articles.
\\
\\
\textbf{DBPedia.} DBPedia is a community project that extracts structured knowledge from Wikipedia and makes it freely available using linked data technologies~\cite{lehmannDBpediaLargescaleMultilingual2015}. The DBPedia dataset for HTC\footnote{\url{https://www.kaggle.com/danofer/dbpedia-classes}} is used as a reference dataset in many state-of-the-art publications~\cite{joulinBagTricksEfficient2016, yangXLNetGeneralizedAutoregressive2020, minaeeDeepLearningBased2020} on text classification. Overall, the dataset contains the introductions of $337,739$ Wikipedia articles, of which $240,942$ are pre-assigned to the training dataset and $60,794$ to the test dataset. Per article, the dataset contains a description of on average 102 words and three one-class label per hierarchy level ($L_1$, $L_2$, $L_3$). Table~\ref{tab:dataset-hierarchy} shows the number of classes on each level of the DBPedia dataset hierarchy and indicates that all texts are assigned to a class on all levels, which means that the labels are \textit{full depth}. Training a differentially private HTC model on a dataset like DBPedia prevents leaking information about participating institutions and people if the underlying encyclopedia is not public.

\section{Experimental Setup}
\label{sec:evaluation:setup}
For our experiments we split the datasets into training, validation and test data. Training data is used to learn the model parameters (i.e., weights), validation data to check the goodness of training hyperparameters and test data is used to assess generalization and real-world performance. Before target and attack model training, so called hyperparameters have to be set manually before training (e.g., learning rate, batch size). We used Bayesian hyperparameter optimization for all target model experiments to ensure that we found good hyperparameters that yield high accuracies on the respective models and data. Bayesian Optimization is more efficient than grid search since it considers past trials during the hyperparameter search. An overview of all hyperparameters, dataset size for training, validation and test, and the overall $\eps$ per training is provided in Table~\ref{tab:hyp}. For the attack model we reused the original hyperparameters of Nasr et al.~\cite{nasrComprehensivePrivacyAnalysis2018} which already performed well. 
The majority of experiments were conducted on EC2\footnote{\url{https://aws.amazon.com/ec2/}} GPU optimized instances of type \enquote{p3.8xlarge} with the \enquote{Deep Learning AMI} machine image, building on a Linux~$4.14$ kernel, Python~$3.6$ and TensorFlow~$2.2$.

\begin{table*}[ht!]
\centering
\caption{Hyperparameters and composed \eps~per model and dataset. The hyperparameters were set with Bayesian optimization.}
 \label{tab:hyp}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{}} & \multicolumn{3}{c|}{BestBuy} & \multicolumn{3}{c|}{Reuters} & \multicolumn{3}{c}{DBPedia} \\ \cline{3-11} 
\multicolumn{2}{c|}{} & BoW & CNN & Transformer & BoW & CNN & Transformer & BoW & CNN & Transformer \\ \hline
\multirow{2}{*}{learning rate} & Orig. & $0.001$ & $0.001$ & $0.005$ & $0.001$ & $0.001$ & $0.005$ & $0.001$ & $0.001$ & $0.005$ \\ \cline{2-11} 
 & DP & $0.01$ & $0.001$ & $0.015$ & $0.008$ & $0.001$ & $0.005$ & $0.016$ & $0.001$ & $0.01$ \\ \hline
\multirow{2}{*}{batch size} & Orig. & $32$ & $32$ & $32$ & $32$ & $32$ & $32$ & $32$ & $32$ & $32$ \\ \cline{2-11} 
 & DP & $64$ & $64$ & $64$ & $64$ & $64$ & $32$ & $64$ & $64$ & $32$ \\ \hline
clipping norm $\mathcal{C}$ & DP & $0.19$ & $1.48$ & $2.07$ & $0.33$ & $6.28$ & $12.86$ & $0.03$ & $0.21$ & $1.6$ \\ \hline
microbatch size & DP & $1$ & $1$ & $1$ & $1$ & $1$ & $4$ & $1$ & $1$ & $4$ \\ \hline
\multirow{4}{*}{$\epsilon$} & $z=0.1$ & $30,253$ & $33,731$ & $5,902$ & $2,048$ & $1,091$ & $21,597$ & $4,317$ & $6,414$ & $24,741$ \\ \cline{2-11} 
 & $z=0.5$ & $11.5$ & $11.1$ & $6.58$ & $4.19$ & $4.11$ & $4.4$ & $5.1$ & $6.29$ & $4.88$ \\ \cline{2-11} 
 & $z=1.0$ & $1.51$ & $1.38$ & $1.04$ & $0.79$ & $0.79$ & $0.77$ & $0.87$ & $0.96$ & $0.81$ \\ \cline{2-11} 
 & $z=3.0$ & $0.26$ & $0.5$ & $0.29$ & $0.22$ & $0.22$ & $0.22$ & $0.2$ & $0.21$ & $0.21$ \\ \hline
\multicolumn{2}{c|}{Training records} & \multicolumn{3}{c|}{$41,625$} & \multicolumn{3}{c|}{$651,585$} & \multicolumn{3}{c}{$240,942$} \\ \hline
\multicolumn{2}{c|}{Validation records} & \multicolumn{3}{c|}{$4,626$} & \multicolumn{3}{c|}{$72,399$} & \multicolumn{3}{c}{$36,003$} \\ \hline
\multicolumn{2}{c|}{Test records} & \multicolumn{3}{c|}{$5,139$} & \multicolumn{3}{c|}{$80,443$} & \multicolumn{3}{c}{$60,794$} \\ \hline

\end{tabular}
\end{table*}

In all experiments we assume that the data owner would also want converging target models even when training with DP. Thus, all HTC models leverage early stopping with a patience of $3$ epochs to terminate the training process before overfitting. Furthermore, we set the DP parameter $C$ (i.e., the sensitivity $\Delta f$) in our experiments to the median of the norms of the unclipped gradients over the course of original training as suggested by Abadi et al.~\cite{abadiDeepLearningDifferential2016}. For all executions of the experiment, CDP noise is sampled from a Gaussian distribution (cf.~Definition~\ref{def:dp:gauss}) with scale $\sgm=\textit{noise multiplier}~z \times \textit{clipping norm}~\cali{C}$. According to McMahan et al.~\cite{mcmahanGeneralApproachAdding2019}, values of $z\approx 1$ will provide reasonable privacy guarantees. We evaluate increasing noise regimes per dataset by evaluating noise multipliers $z\in\{0.1, 0.5, 1.0, 3.0\}$ and calculate the resulting $\eps$~at a fixed $\dlt=\frac{1}{n}$. 

\section{Evaluation}
\label{sec:evaluation}

% in section~\ref{sec:evaluation:setup}
% in section \ref{sec:evaluation:results}
% in section \ref{sec:evaluation:effect:parameters}

In this section, we first describe the experimental setup. Afterwards, we experimentally assess privacy and utility for the previously formulated HTC models and datasets\footnote{We publish all code and experiment scripts at \url{https://github.com/SAP-samples/security-research-dp-hierarchical-text}.}. Lastly, we present several experiment variations to illustrate the impact of different parameters.
%HTC specific attack model features (subsection~\ref{sec:evaluation:effect:attack}) and the effect of varying different target model training parameters (subsection~\ref{sec:evaluation:effect:target}).

\subsection{Empirical Privacy and Utility}
\label{sec:evaluation:results}

%\todo{Argument: Quantify train test gap, compare for different target models, hypothesize MIA}
\noindent
A theoretic comparison of the CNN, BoW and Transformer models with respect to their robustness towards noise that is introduced by DP is only insightful to a limited extend, since their architectures and pre-training paradigms vary. However, in general the bias-variance trade-off for ANNs allows us to formulate high-level expectations. Simple ANNs will likely be prone to high bias and thus underfit in comparison to larger ANNs. Thus, the BoW model will potentially perform poorer on test data than the CNN or Transformer architecture, even in the presence of pre-training~\cite{ezen20}. In contrast, large ANNs will have high variance and thus require larger amounts of training data to generalize well. Thus, the Transformer model will likely perform poorer on small datasets. In general, the bias decreases and the variance increases with the ANN size~\cite{NMB+19}. In combination with DP, we expect high bias models such as the BoW to be less affected by the introduced noise. Additionally, Transformer models may be negatively affected by gradient explosion when using relu activation functions in combination with DP~\cite{papernot2020tempered}.

%\tc{reporting utility is sub-par -- also our discussion to which extent the resulting classification is useful at all, or not...}
Figure~\ref{fig:utility} states the utility and Figure~\ref{fig:mi} the privacy scores over $\epsilon$ for the three datasets and model architectures. Furthermore, we additionally report the theoretical bound on $Adv$ by Yeom et al.~\cite{yeomPrivacyRiskMachine2018} to allow comparison of the theoretical and the empirical MI advantage. Notably, even if two classifiers were trained with the same noise multiplier $z$, they do not necessarily yield the same DP privacy parameter $\epsilon$ due to differing training epochs until convergence. All corresponding $\epsilon$ values per model and dataset were calculated for $\delta = \frac{1}{|\cali{D}_{target}^{train}|}$ per dataset and are stated in Table~\ref{tab:hyp}. 
\begin{figure*}[ht!]
\captionsetup{justification=centering}
    \centering
        \begin{subfigure}{0.75\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/bestbuy_cleaned_utility.pdf}
        \caption{Target model test accuracy for BestBuy utility over $\epsilon$}
        \label{fig:bestbuy_cleaned_utility}
    \end{subfigure}
    \begin{subfigure}{0.75\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/reuters_utility.pdf}
        \caption{Target model test accuracy for Reuters utility over $\epsilon$}
        \label{fig:reuters_utility}
    \end{subfigure}
    \begin{subfigure}{0.75\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/DBPEDIA_utility.pdf}
        \caption{Target model test accuracy for DBPedia over $\epsilon$}
        \label{fig:dbpedia_utility}
    \end{subfigure}
    \caption{Target model test accuracy per dataset over $\epsilon$.}
    \label{fig:utility}
\end{figure*}

\begin{figure*}[ht!]
\captionsetup{justification=centering}
    \centering
    \begin{subfigure}{0.75\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/bestbuy_cleaned_mi.pdf}
        \caption{MI against BestBuy over $\eps$}
        \label{fig:bestbuy_cleaned_mi}
    \end{subfigure}
    \begin{subfigure}{0.75\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/reuters_mi.pdf}
        \caption{MI against Reuters over $\eps$}
        \label{fig:reuters_mi}
    \end{subfigure}
    \begin{subfigure}{0.75\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/DBPEDIA_mi.pdf}
        \caption{MI against DBPedia over $\eps$}
        \label{fig:dbpedia_mi}
    \end{subfigure}
    \caption{MI AUC, $Adv$ and Bound on MI $Adv$ per dataset $\epsilon$.}
    \label{fig:mi}
\end{figure*}

As expected, the model utility and adversary's success consistently decrease with stronger DP parameters for all models and all datasets. Figure~\ref{fig:bestbuy_cleaned_utility} shows that %\tc{could we have predicted this, by any chance? why didn't we, and collected supportive evidence rather than just some observations?}
for BestBuy the BoW model's utility is the most robust to the introduced noise, while the Transformer model's utility is most sensitive to the introduced noise. This observation becomes most evident when considering the flat accuracy $Acc$ (\textit{blue}), and is in line with our expectation for small datasets formulated at the beginning of this section. The hierarchical utility metrics $F_H$ and $F_{LCA}$ do not decrease as strongly as $Acc$, since they also account for partially correct predictions. Interestingly, for BestBuy, the CNN model's MI metrics in Figure~\ref{fig:bestbuy_cleaned_mi} already reach the baseline level at $\epsilon=33,731$ ($z=0.1$). The large $\epsilon$ points out that with respect to the upper bound a huge privacy loss is occurring (i.e., $e^\epsilon$) and the advantage should also be maximal (i.e., $e^\epsilon-1$~\cite{yeomPrivacyRiskMachine2018}). However, the empirical membership advantage lies far below this theoretical bound. In contrast to the CNN, the MI attack against the BoW and Transformer models is only reaching the baseline at $\epsilon=1$ and $\epsilon=1.5$, respectively.

The results for the Reuters dataset are provided in Figure~\ref{fig:reuters_utility} and \ref{fig:reuters_mi}. Compared to BestBuy, the decrease in model utility on Reuters is smaller for all three HTC models, which can be explained with a significantly higher amount of training examples and a smaller amount of hierarchical classes. The BoW classifier's utility is most robust to the addition of noise to the training process, yet closely followed by the Transformer model. However, the CNN model exhibits the most severe decrease in model utility. Figure~\ref{fig:reuters_mi} indicates that the MI adversary's advantage drops to the baseline level again for very weak DP guarantees of $\epsilon>10^2$ for all models. This behavior can be explained with the high amount of training examples and the smaller amount of hierarchical classes. Therefore, the gap between the empirically measured membership advantage and the upper bound on membership advantage diverge widely. 

For DBPedia in Figure~\ref{fig:dbpedia_utility}, the BoW model is again the most robust, and the Transformer model is least robust to the added noise during the training process, similar to the observations made on the BestBuy dataset. This is in line with our formulated expectations. The only exception are the measured utility metrics for $\epsilon\approx10^{-1}$, for which the BoW model performs worse than the CNN and Transformer model. MI metrics for the DBPedia HTC models are provided in Figure~\ref{fig:dbpedia_mi}. We see that the MI metrics for the BoW and Transformer models drop to the baseline level for very weak DP guarantees, similar to the Reuters models. Therefore, our MI adversary does by far not reach the theoretical upper $Adv$ bound. Notably, the MI metrics for the CNN model do not drop to the baseline level for the considered range for $z$ and resulting $\epsilon$. Hence, the gap between the measured $Adv$ and theoretical upper bound on $Adv$ reaches its lowest value for this model.

Overall, the privacy and utility results support our expectation that the utility of a high bias model such as BoW is less affected by the introduced noise than models with high variance such as Transformer. On the other hand, Transformer models are less prone to the MI attack due to better generalization which has generally been demonstrated aside from MI in related work~\cite{vaswaniAttentionAllYou2017,devlinBERTPretrainingDeep2018}.

\begin{table*}[ht!]
\captionsetup{justification=centering}
\centering
\begin{tabular}{cc|c|c|c|c|c|}
\cline{3-7}
                         &       & $n=41,625$,   & $n=41,625$, & $n=41,625$, & $n=4000$            & $n=400$           \\
                         &       & $14$ epochs  & $50$ epochs & $100$ epochs & $30$ epochs & $30$ epochs \\ \hline
\multicolumn{1}{|c|}{\multirow{4}{*}{$\cali{D}_{target}^{train}$}} & $L_1$ & $99.71\%$ & $99.94\%$ & $99.94\%$ & $99.94\%$ & $98.44\%$ \\ \cline{2-7} 
\multicolumn{1}{|c|}{}   & $L_2$ & $99.20\%$    & $99.86\%$         & $99.92\%$          & $99.44\%$            & $85.16\%$          \\ \cline{2-7} 
\multicolumn{1}{|c|}{}   & $L_3$ & $96.91\%$    & $99.74\%$         & $99.81\%$          & $96.07\%$            & $63.28\%$          \\ \cline{2-7} 
\multicolumn{1}{|c|}{}   & Loss  & $0.18$       & $0.01$            & $0.01$             & $0.30$               & $3.15$             \\ \hline
\multicolumn{1}{|c|}{\multirow{4}{*}{$\cali{D}_{target}^{test}$}}  & $L_1$ & $97.24\%$ & $96.93\%$ & $97.06\%$ & $93.47\%$ & $84.31\%$ \\ \cline{2-7} 
\multicolumn{1}{|c|}{}   & $L_2$ & $95.00\%$    & $94.79\%$         & $94.73\%$          & $87.89\%$            & $59.23\%$          \\ \cline{2-7} 
\multicolumn{1}{|c|}{}   & $L_3$ & $89.32\%$    & $91.11\%$         & $91.35\%$          & $78.53\%$            & $37.76\%$          \\ \cline{2-7} 
\multicolumn{1}{|c|}{}   & Loss  & $0.89$       & $1.60$            & $1.87$             & $2.08$               & $3.97$             \\ \hline
\multicolumn{2}{|c|}{$L_3$ Gap}  & $7.60\%$     & $8.63\%$          & $8.47\%$           & $17.54\%$            & $25.52\%$          \\ \hline
\multicolumn{2}{|c|}{Loss Ratio} & $5.2$        & $160$             & $187$              & $6.93$               & $1.26$             \\ \hline
\multicolumn{2}{|c|}{$Acc_{MI}$} & $53.06\%$    & $53.92\%$         & $54.01\%$          & $64.62\%$            & $75.00\%$          \\ \hline
\end{tabular}
\caption{Per-level accuracies and summarized loss for BestBuy  Transformer network without DP.}
\label{tab:target-model-mods}
\end{table*}

\subsection{Drivers for Attack Performance}
\label{sec:evaluation:effect:parameters}

%It is noticeable that the observed MI accuracies are rather low \todo{Make more conrete/quantify} throughout all experiments. 
Our experiments show that state-of-the-art MI attacks are not very effective when run against the trained HTC models. % TODO more specific, compare with Shokri?!
This leads to the question whether more HTC-specific attacks or less generalizing HTC target models would boost attack performance. In the following subsections, we first validate experimentally that the attack performance does not increase when introducing HTC-specific attack features. Second, we present several means that reduce target model generalization, where we show that especially reducing the number of training examples increases the vulnerability to MI attacks.

\subsubsection{HTC-specific attack model features}
\label{sec:evaluation:effect:attack}

We hypothesize that adapting the MI attack to exploit the hierarchical relation of the classes leads to an increased MI attack performance. Our approach to adapt the MI attack to HTC models is to extract additional attack features from the target model. We choose to evaluate two additional features in the following.

The former is a Boolean feature that we derive by checking if the HTC model's prediction before applying the post-processing step is consistent with the hierarchy of the HTC task. The latter is a scalar feature that is derived by multiplying the probabilities of the node with the highest softmax score on each level. The intuition behind this feature is to calculate a value that states how confident the target model is with the predicted label, since the assigned probability is obviously higher when the model outputs only small probabilities for the other labels. We refer to this attack feature as \textit{prediction confidence}.

We pass the features into the attack model with an additional FCN similar to the loss. We tested the effect of the additional features on all datasets and models. However, the results for this attack variant do not result in a significant change of the considered MI metrics (Figures~\ref{fig:bestbuy_mi_whf} to \ref{fig:dbpedia_mi_whf} in the appendix).

\subsubsection{Reduced Target Model Generalization}
\label{sec:evaluation:effect:target}

Next, we describe four approaches that we formulated to increase the attack model performance by reducing target model generalization in HTC. Each approach is first motivated and then evaluated based on experimental results.

First, we provoke an overfitted target model by training without early stopping for a fixed number of epochs, which is chosen significantly higher than the original number of epochs obtained with early stopping. In doing so, we deliberately force the model to overfit, i.e.,~adapt to the few samples in $\cali{D}_{target}^{train}$ instead of approximating the underlying distribution. We evaluated this approach based on the BestBuy Transformer classifier. Table~\ref{tab:target-model-mods} shows the metrics of the original model in the first column, which converged after 14 epochs. The second and third column reveal the metrics for overfit models, which are trained for 50 and 100 epochs, respectively. As expected, the overfit models achieve a smaller training loss and a higher test loss. However, surprisingly, the achieved test accuracy does not drop compared to the original model, while the training accuracy on $L_3$ increases to over $99\%$. The corresponding attack model accuracies rise from $53.06\%$ to $53.92\%$ and $54.01\%$ respectively. This insignificant change may appear counter-intuitive given the increased loss on $\cali{D}_{target}^{test}$. However, when analyzing the loss distribution of $\cali{D}_{target}^{train}$ and $\cali{D}_{target}^{test}$, we observe that the median losses decrease similarly as depicted in Figure~\ref{fig:loss_dist:orig} and \ref{fig:loss_dist:overfit}. The reason for the high average loss on $\cali{D}_{target}^{test}$ is due to the high loss value of a few outliers. Therefore, the loss ratio is not a consistently good indicator for MI attack effectiveness in practice and rather the accuracy gap should be taken into account.

\begin{figure}[ht!]
\captionsetup{justification=centering}
    \centering
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/loss_boxplots_bestbuy_bert_orig.pdf}
        \caption{Loss on original model after 14 epochs}
        \label{fig:loss_dist:orig}
    \end{subfigure}%
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/loss_boxplots_bestbuy_bert_overfit100.pdf}
        \caption{Loss on overfit model after 100 epochs}
        \label{fig:loss_dist:overfit}
    \end{subfigure}
    \caption{Loss distribution of members and non-members for BestBuy. Each boxplot is on a log scale depicting outliers (black), median (green) and mean (red) of the respective distribution.}
    \label{fig:loss_dist}
\end{figure}

\begin{figure*}[h]
\captionsetup{justification=centering}
    \centering
        \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/bestbuy_bow_ratio.pdf}
        \caption{Relation between the records/levels ratio and attack advantage for BestBuy}
        \label{fig:bestbuy_cleaned_ratio}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/reuters_bow_ratio.pdf}
        \caption{Relation between the records/levels ratio and attack advantage for Reuters}
        \label{fig:reuters_ratio}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/dbpedia_bow_ratio.pdf}
        \caption{Relation between the records/levels ratio and attack advantage for DBPedia }
        \label{fig:dbpedia_ratio}
    \end{subfigure}
    \caption{Attack model advantage over ratio of records per hierarchy for an overall number of $\{0.25, 0.5, 0.75, 1\}\times n$ training records.}
    \label{fig:ratio}
\end{figure*}

Second, we reduce the number of training examples in $\cali{D}_{target}^{train}$. With this adaption, the hierarchical classifier should not generalize as well as the original classifier due to two reasons. First, the training dataset is less representative of the problem domain, and second, underrepresented classes contain even fewer examples. % should we explain this?
We again evaluate this approach based on the BestBuy transformer classifier, which originally contains $n=41,625$ training examples. Training the classifier with only $10\%$ of the training examples indeed leads to worse generalization with a maximum train-test gap of $17.54\%$ on the third level as shown in Table~\ref{tab:target-model-mods}. The trained attack model for this variation converged at $64.62\%$ accuracy, which is a significant increase compared to the original target model. Further reducing the training data to $n=400$ examples reduces the target model performance even more, with a maximum train-test gap of $25.52\%$ on the third level, as evident from Table~\ref{tab:target-model-mods}. For this target model with $n=400$, we observe an attack accuracy of $75\%$. In conclusion, reducing the number of training examples results in a significant MI attack improvement in comparison to changing the attack model features.

Third, we increase the number of hierarchy levels in the data, resulting in a more complex HTC task, which we again hypothesize to lead to worse generalization. Moreover, additional hierarchy levels lead to additional classification outputs and therefore additional attack features, which might further boost attack performance. And indeed, when increasing the number of levels from three to seven for the BestBuy BoW classifier, the corresponding MI attack accuracy rises from $56.15\%$ to $57.07\%$. To ensure that this effect was caused by noise, we also reduced the number of levels to one, resulting in an attack accuracy of $51.38\%$. This shows that an increased (decreased) number of hierarchy levels leads to higher (lower) attack performances.

Interestingly, when combining the effects of changing the number of hierarchy levels and decreasing the number of training examples, we made the observation that the ratio of the number of training examples to levels in the HTC task has an direct influence on the MI attack performance. We first noted this effect for BestBuy and then validated if we can also see it for the other datasets. The results confirm our expectations and are shown in Figure \ref{fig:ratio}.

Finally, we train the hierarchical classifier from scratch, without leveraging pre-trained weights to initialise the model. We hypothesize that this classifier variation might be more vulnerable to MI attacks, since a model without pre-training might tend to memorize more information about $\cali{D}_{target}^{train}$. Training the original BestBuy Transformer classifier from scratch did not converge to a useful HTC model, with only $18\%$ accuracy on the first level. This effect can be explained by the relatively small amount of training data compared to the large corpora the Transformer model is usually pre-trained on. The issue can be overcome by replacing the BERT-Base layers with BERT-Tiny layers, since tiny layer contain fewer weights to train. The hierarchical BERT-Tiny classifier trained from scratch yields a model with $75.17\%$ flat $Acc$. The trained attack model for this variation converged at $55.04\%$ accuracy, which is $\approx2\%$ higher than the attack on the original target model. This relatively small increase reveals that the use of pre-trained weights for the target models is not the reason for the relatively poor attack performance. 
